ClickBAIT-v2: Training an Object Detector in Real-Time

Modern deep convolutional neural networks (CNNs) for image classification and object detection are often trained offline on large static datasets. Some applications, however, will require training in real-time on live video streams with a human-in-the-loop. We refer to this class of problem as time-ordered online training (ToOT). These problems will require a consideration of not only the quantity of incoming training data, but the human effort required to annotate and use it. We demonstrate and evaluate a system tailored to training an object detector on a live video stream with minimal input from a human operator. We show that we can obtain bounding box annotation from weakly-supervised single-point clicks through interactive segmentation. Furthermore, by exploiting the time-ordered nature of the video stream through object tracking, we can increase the average training benefit of human interactions by 3-4 times.

==> software_architecture.tex <==
% \ervin{This section definitely appeals more to a systems/engineering audience than an algorithms one. It will definitely stay for ArXiV release - but consider removing in liew of e.g. more datasets/benchmarks for CVPR.}
\subsection{Application and Requirements}

%We specifically target the application
We consider the challenge of training a UAS to recognize and geo-tag objects of interest within its field of view and plotting the results on a map for human operators. We add the stipulation that our system should be target-agnostic, and that \textit{training of the recognizer will take place while the system is operational.} We design this system subject to the following requirements:
\begin{itemize}
\item Recognizer must be able to classify at least two categories, \ie{} target detected and target not detected.
\item Recognitions should happen in real-time, \ie{} >5 times per second on a video feed from the UAS' camera.
\item Recognized targets should be highlighted (localized) in their images when sent to the operator.
\item If the operator does not agree with the classification result of the recognizer, the operator can initiate a training round on that particular frame.
\item The newly updated model should immediately be used for the next recognition.
\item All computational tasks associated with training and recognition must be performed onboard the UAS itself.
\end{itemize}

\subsection{System Design}

Figure~\ref{fig:diagram} shows the system design. The training system has two main components: the \textit{Ground Station} to interact with the human operator, and the \textit{UAS} that houses the CNN and performs recognition and training.

\begin{figure} \centering
    \includegraphics[width=0.80\linewidth]{system_diagram}
    \caption{Diagram of both UAS and ground part of training system.}
    \label{fig:diagram}
\end{figure}

\subsubsection{Ground Station}
\label{sec:groundstation}

The Ground Station is a Web application backed by MongoDB, which receives, stores, and displays classification results. A websocket connection is maintained between the Ground Station and the UAV, over which downsized images (224x224 pixels, approx. 20 KB) and classification results are sent down, and training commands are sent up. The user interface (Figure~\ref{fig:userinterface}) displays the image stream, overlaid with a Class Activation Map~\cite{Zhou2016} showing the user where the object of interest is. Recognition results are also plotted on a map in real-time based on the GPS location of the UAS and can be filtered to show only positive results. For all incoming data points, both the images and the results are stored for future review.

\begin{figure}[h] \centering
    \includegraphics[width=0.80\linewidth]{ui}
    \caption{Training and Recognition User Interface. The right panel shows the current recognition result and the training interface, while the left shows a real-time map of results.}
    \label{fig:userinterface}
\end{figure}

The operator can tag the current image for training by clicking on the positive (green) or negative (red) buttons under the viewport showing the camera feed in the top-right corner.
This triggers a user interaction, sending the user's tag and the corresponding back to the UAS where it initiates a training round, \ie{}  one gradient update. Clicking on the image itself sends the cursor position along with the training image and a positive tag; this is used for localized learning (described in the following section). 

\subsubsection{UAS}
The UAS is a small, commercial off-the-shelf (CoTS) quadrotor~\footnote{3D Robotics Solo}, with a payload capacity of 700g. The payload consists of a gimbal-mounted GoPro camera with altered rectilinear optics, and an NVIDIA Jetson TX1 embedded GPU computing module. Video from the camera is streamed to the quadrotor's internal CPU, which encodes the video stream as RTP\footnote{RTP Payload Format for H.264 Video. https://tools.ietf.org/html/rfc6184} over UDP and sends the stream both to the pilot, to aid in aiming the camera, and to the learning system.

\subsubsection{Learning System}
\label{sec:learningsystem}
On the computing module runs the recognition and training system, based on the TensorFlow~\cite{Abadi2015} GPU-accelerated framework. For the CNN, we use the GoogLeNet+GAP formulation suggested in~\cite{Zhou2016}, an augmented GoogLeNet~\cite{Szegedy2014}, for its relatively good performance on ImageNet, lightweight nature both in size of weights as well as execution time, and its ability to provide simple localization based on class activation maps. Class activation mapping through global average pooling~\cite{Zhou2016} is chosen over bounding box regression methods such as~\cite{Redmon2015} so that the human operator has the option of weakly supervising, \ie tag positive or negative, each frame. The computing module continuously grabs the most recent frame from the video stream, performs a single forward propagation using this image, and sends both the image and the class activation map to the Ground Station. If a human-tagged image is received from the Ground Station, the compute module stores the image and tags in a database, and subsequently executes a training step (forward propagation, backwards propagation, weights update). The stored images can be used to generate the next training batch (Section~\ref{sec:experiments}). The updated weights are immediately used to evaluate the next grabbed frame from the video stream, and any improvements are recognizable by the operator, as shown in Algorithm~\ref{alg:videoingestion}.

\begin{algorithm}
\caption{Training From a Video Feed}\label{alg:videoingestion}
\begin{algorithmic}[1]
% \Procedure{}{$a,b$}\Comment{The g.c.d. of a and b}
\While{insufficient model performance}
  \State $v \gets $ fetchFromCamera()
  \State $v_{user} \gets $forwardProp($v$)
  \State showUser($v_{user}$)
  \State $u, tag \gets $ getUserInput()
    \If{$u = 1$} \Comment{If user input exists}
    \State $B \gets $createMiniBatch($v, tag$)
    \State forwardProp($B$)
    \State backProp()
    \State weightsUpdate()
    \State storeInHistoryDB($v, tag$)
    \EndIf
\EndWhile
\State \textbf{return} 
\end{algorithmic}
\end{algorithm}

